Vision-Based Real-Time Indoor Positioning System for Multiple Vehicles

We propose a novel external indoor positioning system that computes the position and orientation of multiple model-scale vehicles. For this purpose, we use a camera mounted at a height of 3.3m and LEDs attached to each vehicle. We reach an accuracy of about 1.1 cm for the position and around 0.6 {\deg} for the orientation in the mean. Our system is real-time capable with a soft deadline of 20 ms. Moreover, it is robust against changing lighting conditions and reflections.

==> tables/AccuracyCompare.tex <==
\begin{tabular}{ l | c c c | c c}
	 & Ratosi & \multicolumn{2}{c|}{Faessler 2014} & \multicolumn{2}{c}{our System}  \\
				 & 2018   & \textcolor{darkgray}{\unit[1]{m}} & \unit[3]{m} & \textcolor{black}{Exp.} & \textit{Sim.}\\ 
	Position [\unit{cm}] & & &\\
	\hline
 	Mean & $2.6$ & \textcolor{darkgray}{$0.74$} & $\sim 5.4$ & \textcolor{black}{$\mathbf{1.11}$}  & $\mathit{0.45}$\\
 	Max  & $7.62$ & \textcolor{darkgray}{$3.28$} &  $\sim 8.7$ & \textcolor{black}{$\mathbf{3.25}$} & $\mathit{0.57}$\\
 	Std dev &  $\mathbf{0.51}$& \textcolor{darkgray}{$0.46$} & - & \textcolor{black}{$0.66$} & $\mathit{0.04}$\\
 	
 &&&&&\\
 	Orientation [\unit{\degree}]  & & & &  \\
 	\hline
 	Mean  & $0.9$ & \textcolor{darkgray}{$0.79$} & $\sim 1.25$ & \textcolor{black}{$\mathbf{0.63}$} & $\mathit{0.26}$\\
 	Max   & $\mathbf{1.4}$ & \textcolor{darkgray}{$3.37$} & $\sim 4.3$ & \textcolor{black}{$2.25$} & $\mathit{0.88}$\\
 	Std dev & $\mathbf{0.1}$ &  \textcolor{darkgray}{$0.41$} & - & \textcolor{black}{$0.52$} & $\mathit{0.15}$\\
\end{tabular}
